Efficient Speed Planning for Autonomous Driving in Dynamic Environment with Interaction Point Model

Safely interacting with other traffic participants is one of the core requirements for autonomous driving, especially in intersections and occlusions. Most existing approaches are designed for particular scenarios and require significant human labor in parameter tuning to be applied to different situations. To solve this problem, we first propose a learning-based Interaction Point Model (IPM), which describes the interaction between agents with the protection time and interaction priority in a unified manner. We further integrate the proposed IPM into a novel planning framework, demonstrating its effectiveness and robustness through comprehensive simulations in highly dynamic environments.

==> backup_copy <==
\author{
\begin{tabular}{@{}c@{}}
Yingbing Chen$^{1}$, 
Ren Xin$^{1}$,
Jie Cheng$^{1}$, \textit{Student Member, IEEE}, \\ 
Qingwen Zhang$^{1}$, \textit{Student Member, IEEE},
Xiaodong Mei$^{1}$, \textit{Student Member, IEEE}, \\
Ming Liu$^{1,2}$, \textit{Senior Member, IEEE},
and Lujia Wang$^{1}$, \textit{Member, IEEE}
\end{tabular}}

\thanks{Manuscript received: March 29, 2022; Revised July 14, 2022; Accepted September 4, 2022. This paper was recommended for publication by Editor Tamim Asfour upon evaluation of the Associate Editor and the reviewers' comments.
This work was supported by Guangdong Basic and Applied Basic Research Foundation, under project 2021B1515120032, Zhongshan Science and Technology Bureau Fundunder project 2020AG002, and Project of Hetao Shenzhen-Hong Kong Science and Technology Innovation Cooperation Zone(HZQB-KCZYB-2020083), awarded to Prof. Ming Liu. (\textit{Corresponding author: Ming Liu.})} %Use only for final RAL version

\thanks{$^{1}$Yingbing Chen, Ren Xin, Jie Cheng,  Qingwen Zhang, Xiaodong Mei, and Lujia are with Robotics Institute, the HKUST, Hong Kong SAR, China, the Clear Water Bay Institute of Autonomous Driving, and also with the Systems Hub, HKUST (GZ). {\tt\footnotesize \{ychengz\}@connect.ust.hk}.}%

\thanks{$^{2}$Ming Liu is with Robotics Institute, the HKUST, Hong Kong SAR, China, the HKUST (Guangzhou), Nansha, Guangzhou, 511400, Guangdong, China, and also with the HKUST Shenzhen-Hong Kong Collaborative Innovation Research Institute, Futian, Shenzhen. {\tt\footnotesize eelium@ust.hk}.}%
